Toward Gender-Inclusive Coreference Resolution

Correctly resolving textual mentions of people fundamentally entails making inferences about those people. Such inferences raise the risk of systemic biases in coreference resolution systems, including biases that can harm binary and non-binary trans and cis stakeholders. To better understand such biases, we foreground nuanced conceptualizations of gender from sociology and sociolinguistics, and develop two new datasets for interrogating bias in crowd annotations and in existing coreference resolution systems. Through these studies, conducted on English text, we confirm that without acknowledging and building systems that recognize the complexity of gender, we build systems that lead to many potential harms.

==> bias.tex <==
In this section, we analyze several ways in which harmful biases can and do enter into the machine learning lifecycle of coreference resolution systems (per \autoref{fig:lifecycle}).
Two stages discussed by \citet{vaughan2019fairness} that we exclude are Training Process and Deployment.
It is rare (as they observed as well) for training processes (especially in batch learning settings) to lead to bias, and the same appears to be the case here.
We do not consider the ``Deployment'' phase, because we are not aware of deployed coreference resolution systems to test; except, perhaps, those embedded in other systems, which we discuss in the context of testing (\autoref{sec:testing}).



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "coref"
%%% End: 


==> datax.tex <==
In coreference resolution, as in most NLP data collection settings, one typically first collects raw text and then has human annotators label that text.
Here, we consider biases that arise due to the selection of what texts to have annotated.
As an example, if a data curator chooses newswire text from certain sources as source material, xey are unlikely to observe singular uses of \pron{they} which, for instance, was only added to the Washington Post style guide in late 2015 \citep{wapo2015they} and by the Associated Press Stylebook in early 2017 \citep{ap2017they}.
If the raw data does not contain certain phenomena, this fundamentally limits all further stages in the machine learning lifecycle (a system which has never seen ``hir'' is unlikely to even know it's a pronoun, much less how to link it; indeed the off-the-shelf tokenizer we used often failed to separate ``xey're'' into two tokens, as it does for ``they're'').

To analyze the possible impact of input data, we consider our thirteen coreference datasets, and count how many instances of different types of pronouns are used in the raw data.
We focus on \pron{she}, \pron{he}, and \pron{they} pronouns (in all their morphological forms); we additionally counted several neopronoun forms (\pron{hir}, \pron{xey} and \pron{ey}) and found no occurrences nor their morphological variances.\footnote{There was one instance of ``hir'' but that was a almost certainly typo for ``his'' (given the context), and several instances of ``ey'' used a contractions for plural \pron{they} in transcripts of spoken English.}
In the case of \pron{they}, we distinguish between four uses of \pron{they}: plural, singular, quantified (e.g., ``Every student handed in their homework''), and non-human (referring, for instance, to a set of boxes).
To achieve this, we annotated 100 examples uniformly at random by hand from OntoNotes \cite{onto5}.
Furthermore, we compare to the raw counts in a 2015 dump from some of Reddit discussion forum\footnote{From \url{https://www.reddit.com/r/datasets/comments/3bxlg7/i_have_every_publicly_available_reddit_comment/}}, and also limited to the \texttt{genderqueer} subforum.
We additionally a new dataset for study, GICoref, described below in \autoref{sec:gicoref}.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{datax_g1.png}

    \includegraphics[width=12cm]{datax_g2.png}

    \caption{\label{tab:datax} (Top) For each dataset under consideration, the fraction of pronouns with different forms. Only our dataset (GICoref) and the genderqueer subreddit include neopronouns. (In the case of GAP, there \emph{are} some occurrences of \pron{they}, but they are never considered targets for coreference and so we exclude them from these counts.) (Bottom) For three datasets, the fraction (out of 100 annotated) of each \emph{they} into one of the four usage cases.}
\end{figure}

The results of this analysis are in \autoref{tab:datax}, including results on our new dataset, \newdataset.
Overall, the examples used in the documentation of each of these datasets focuses entirely on binary gendered pronouns, generally with many more \pron{he} examples than \pron{she} examples. Only the older datasets (MUC7 and Zh-PB3) include any examples of \pron{they}, some of which are in a quantified form.
Although the examples in annotation guidelines (or papers) are insufficient to fully tell what annotations were intended by the authors, they do provide a sense of what may have been top of mind in dataset construction.


\subsubsection{New Dataset: Gender Inclusive Coreference} \label{sec:gicoref}

In order to make progress on gender inclusive coreference resolution, we introduce a new dataset, \newdataset.
This dataset is collected for the purpose to evaluate current coreference resolution models in the contexts where a broader range of gender identities are reflected, where linguistic examples of genderfluidity are encountered, where non-binary pronouns are used, and where misgendering happens.
In comparison to \citep{zhao2018gender} and \cite{rudinger2018gender} (as well as in contrast to our \MAP dataset), we focused on \emph{naturally} occurring data, but sampled specifically to surface more gender-related phenomena than may be found in, say, the Wall Street Journal.

The \newdataset dataset consists of 95 documents from three types of sources: articles on English Wikipedia about people with non-binary gender identities, articles from LGBTQ periodicals, and fan-fiction stories from Archive Of Our Own (with the respective author's permission). Each author manually annotated each of these documents (additional detail of the dataset can be found in the accompanying datasheet), and then we jointly adjudicated the results. To reduce annotation time, any article that was substantially longer than 1000 words (pre-tokenization) was trimmed at the 1000th word.\footnote{There are four documents we accidentally trimmed at the 2000th word and so we keep the longer version of them with 2000 words in the dataset.} This data includes many examples of people who use pronouns other than \pron{she} or \pron{he}, people who are genderfluid and whose name or pronouns changes through the article, people who are misgendered, and people in relationships that are not heteronormative. Two example annotated documents, one from Wikipedia, and one from Archive of Our Own, are provided in \autoref{ex:wiki} and \autoref{ex:ao3} respectively.

Although the majority of the examples in the dataset are set in a Western context, we endeavored to have a broader range of experiences represented. We included articles about people who are gender non-conforming, but where sociological notions of gender mismatch the general sex/gender/sexuality taxonomy of the West. This includes people who identify as \emph{hijra} (Indian subcontinent), \emph{phuying} (Thailand, sometimes referred to as \emph{kathoey}), \emph{muxe} (Oaxaca), \emph{two-spirit} (Americas), \emph{fa'afafine} (Samoa) and \emph{m\=ah\=u} (Hawaii) individuals.

%\begin{table}
%  \tablesize\centering
%  \begin{tabular}{cc} % |b{7cm}|m{6cm}|}
%    \begin{tabular}[b]{lcccc}
%    \toprule
%%    &&&& \multicolumn{4}{c}{\pron{they}} \\
%    & \pron{she}
%    & \pron{he}
%    & \pron{neo}
%    & \pron{they}
%%    & \pron{-sp}
%%    & \pron{-qi}
%%    & \pron{-pl}
%%    & \pron{-nh}
%    \\
%    \midrule %                          SHE       HE     NEO       -SP       -Q       -P      -NH
%    \corpusname{LDC2001T02}         &  13.9  &  47.0  &  ~~0.0 &  39.1 \\
%    \corpusname{LDC2003T13}         &  12.2  &  53.4  &  ~~0.0 &  34.4 \\
%    \corpusname{LDC2005T09}         & ~~8.9\!&  57.0  &  ~~0.0 &  34.1 \\
%    \corpusname{LDC2005T33}         & ~~8.3\!&  48.7  &  ~~0.0 &  43.0 \\
%    \corpusname{LDC2006T06}         &  17.3  &  41.5  &  ~~0.0 &  41.2 \\
%    \corpusname{LDC2009T10}         & ~~2.4\!&  53.3  &  ~~0.0 &  44.2 \\
%    \corpusname{LDC2009T26}         &  11.7  &  19.9  &  ~~0.0 &  68.4 \\
%    \corpusname{LDC2013T12}         &  25.5  &  43.3  &  ~~0.0 &  31.2 \\
%    \corpusname{LDC2013T19}         &  12.0  &  47.6  &  ~~0.0 &  40.4 \\
%    \corpusname{LDC2017T08}         &  35.7  &  42.9  &  ~~0.0 &  21.4 \\
%    \corpusname{LDC2017T10}         &  10.4  &  39.7  &  ~~0.0 &  49.9 \\
%    \corpusname{GAP}                &  48.8  &  42.6  &  ~~0.0 &  ~~8.6\!\\
%    \corpusname{QB}                 &  18.9  &  76.3  &  ~~0.0 &  ~~4.8\!\\
%%    \bottomrule
%%    reddit                          &  14.2  &  36.5  & ?      &  49.3 \\
%%    \midrule
%    reddit/gq                       &  16.2  &~~6.1\!& ~~4.6\!&  73.1 \\  % terf-ey, slang-ey, oh em gee
%    % original counts for reddit/gq
%    % 779 THEY
%    % 186 SHE
%    % 70 HE
%    % 133 NBIN
%    % but of those NBIN, ~43.2% are THEY in disguise, and 18.2\% are ADJ forms, so add 57 to THEY and remove 24 from NBIN
%    % 836 THEY --> 73.1%
%    % 186 SHE  --> 16.2%
%    % 70 HE    -->  6.1%
%    % 52 NBIN  -->  4.6%
%%    \midrule
%    \newdataset                     &  20.2  & 26.7  &  17.6  &  35.5 \\ % checked and all are legit
%    % for newdataset:
%    % 1425    35.5    35.5    THEY
%    % 1070    26.7    62.3    HE
%    % 811     20.2    82.5    SHE
%    % 293     7.3     89.8    ZE
%    % 171     4.2     94.1    EY
%    % 115     2.8     97      NE
%    % 64      1.5     98.6    XEY
%    % 55      1.3     100     AE      
%    \bottomrule
%%    \corpusname{LDC2001T02}         &  14.5  &  42.5  &  43.0  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2003T13}         & ~~7.2  &  51.8  &  41.0  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2005T09}         & ~~8.6  &  53.2  &  38.2  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2005T33}         & ~~8.2  &  48.6  &  43.2  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2006T06}         &  16.1  &  38.5  &  45.4  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2009T10}         & ~~0.8  &  53.0  &  46.2  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2009T26}         &  11.7  &  19.9  &  68.4  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2013T12}         &  23.3  &  46.5  &  30.2  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2013T19}         &  11.8  &  46.7  &  41.5  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2017T08}         &  46.0  &  40.0  &  14.0  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    \corpusname{LDC2017T10}         &  10.4  &  39.7  &  49.9  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    GAP                             &  42.5  &  48.8  & ~~8.7  &  ~~0.0  &  ????  &  ????  &  ????  \\
%%    QB                              &  18.3  &  75.3  & ~~6.4  &  ~~0.0  &  ????  &  ????  &  ????  \\    
%  \end{tabular} &
%  \begin{tabular}[b]{lcccc} 
%    \toprule
%    & \multicolumn{4}{c}{\pron{they-}} \\
%    & \pron{sp} & \pron{qi} & \pron{pl} & \pron{nh} \\
%    \midrule
%    \corpusname{LDC2013T19} & ~~0\!&  28 &  34 &  38 \\
%%    \midrule
%%    reddit                  & ~~0 &  ~~0 &  ~~0 &  ~~0 \\
%    reddit/gq               &  10 &   43 &   12 &   35 \\
%%    \midrule                  sp     qi     pl     nh
%    \newdataset             &  53 &   13 &   21 &   13 \\
%    \bottomrule
%  \end{tabular} 
%  \end{tabular}
%\end{table}
  
 


%\hal{TODO}: talk about \citep{rudinger2018gender} \hal{next section} and \citep{zhao2018gender} on constructing datasets for testing systems


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "coref"
%%% End: 


==> feedback.tex <==
The final sources of bias we consider are feedback loops: essentially, when the bias from a coreference system feeds back on itself, or onto other coreference systems.

The most straightforward way in which this can happen is through coreference resolution systems that engage in \emph{statistically biased} active learning (or bootstrapping) techniques.\footnote{Here, the overloading of ``bias'' is unfortunate. By ``statistically biased,'' we mean bias in the technical sense that of a learning system that even in the limit of infinite data does not infer the optimal model, a fundamentally different concept from the sort of ``bias'' we consider in the rest of this paper.}
Active learning for coreference has been popular since the early 2000s, perhaps largely because coreference annotation is quite costly.
Considering the approaches used in dominant papers, the active learning algorithms used are not statistically unbiased \citep{ng2003bootstrapping,laws2012active,miller2012active,sachan2015active,guha2015removing}.

Another example is the use of external dictionaries that encode world knowledge that is potentially useful to coreference resolution systems.
The earliest example we know of that uses such knowledge sources is the end-to-end machine learning approach of \citet{daume05coref}, which found substantial benefit by using mined mappings between names and professions to help resolve named entities like ``Bill Clinton'' to nominals like ``president'' (later examples include that of \citet{rahman2011coreference} and \citet{bansal2012coreference}, who found less benefit from a similar approach).

More frequent is the almost ubiquitous use of ``name lists'' that map names (either full names or simply given names) to ``gender.''
And the most frequently used of these is the resource developed by \citet{bergsma2006bootstrapping} (henceforth, B+L), in which a large quantity of text was processed with ``high precision'' anaphora resolution links to associate names with ``genders.''
The process specifically mapped names to \emph{pronouns}, from which gender (presumably an approximation of referential gender) was inferred.
This leads to a resource that pairs a full name or name substring (like ``Bill Clinton'') counts for identified coreference with \pron{he} (8150, 97.7\%), \pron{she} (70, 0.8\%), \pron{it} (42, 0.5\%) and \pron{they} (82, 1\%); these are referred to, respectively, as ``male'', ``female'', ``neuter'' and ``plural,'' and seemingly largely used as such in work that leverages this resource.
We focus on this resource only because it has become ubiquitous, both in coreference resolution and in gender analysis in NLP more broadly.

\begin{table}
  \centering\tablesize
  \begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{5}{c}{\textbf{``Gender'' \% Likelihood}} & \\
    \cline{2-6}
    & \textbf{Masc}
    & \textbf{Fem}
    & \textbf{Neut}
    & \textbf{Plur}
    & \textbf{Unk}
    & \textbf{\textcolor{black!50!white}{count}}
    \\
    \midrule
    she  	& 27	& 41	& 18	& 0	& 14 	& \textcolor{black!50!white}{22} \\
    he   	& 64	& 7	& 7	& 0	& 22 	& \textcolor{black!50!white}{14} \\
    \midrule
    they & 39 & 32 & 12 & 5 & 12 & \textcolor{black!50!white}{41} \\
    ze & 22 & 33 & 33 & 11 & 0 & \textcolor{black!50!white}{9} \\
    they$\vee$she & 25 & 50 & 25 & 0 & 0 & \textcolor{black!50!white}{4} \\
    s/he & 0 & 0 & 50 & 0 & 50 & \textcolor{black!50!white}{2} \\
    they$\wedge$she & 50 & 0 & 0 & 0 & 50 & \textcolor{black!50!white}{2} \\
    all/any & 50 & 50 & 0 & 0 & 0 & \textcolor{black!50!white}{2} \\
    xe & 50 & 0 & 0 & 0 & 50 & \textcolor{black!50!white}{2} \\
    ey & 50 & 0 & 0 & 0 & 50 & \textcolor{black!50!white}{2} \\
    v & 100 & 0 & 0 & 0 & 0 & \textcolor{black!50!white}{1} \\
    ae & 0 & 100 & 0 & 0 & 0 & \textcolor{black!50!white}{1} \\
    ne & 100 & 0 & 0 & 0 & 0 & \textcolor{black!50!white}{1} \\
    ze$\wedge$she & 0 & 0 & 100 & 0 & 0 & \textcolor{black!50!white}{1} \\
%    they	& 38	& 32	& 12	& 3	& 15 	& \textcolor{black!50!white}{34} \\
%    ze  	& 24 	& 38	& 38	& 0	& 0 	& \textcolor{black!50!white}{8} \\
%  they$\vee$she	& 25	& 50	& 25	& 0	& 0 	& \textcolor{black!50!white}{4} \\
%they$\wedge$she	& 50	& 0	& 0	& 0	& 50 	& \textcolor{black!50!white}{2} \\
%    s/he	& 0	& 0	& 50	& 0	& 50 	& \textcolor{black!50!white}{2} \\
%    all/any	& 50	& 50	& 0	& 0	& 0 	& \textcolor{black!50!white}{2} \\
%    ey  	& 100	& 0	& 0	& 0	& 0 	& \textcolor{black!50!white}{1} \\
%    xe  	& 100	& 0	& 0	& 0	& 0 	& \textcolor{black!50!white}{1} \\
%    v   	& 100	& 0	& 0	& 0	& 0 	& \textcolor{black!50!white}{1} \\
%\textbf{non-binary}& 38	& 31	& 16	& 2	& 13 	& \textcolor{black!50!white}{55} \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:bergsmawikinb} For non-binary individuals in our Wikipedia sample (for whom Wikipedia attests current pronouns), a confusion matrix between the pronoun(s) they use (rows) and the inferred gender of their name (based on \citep{bergsma2006bootstrapping}) in columns (where Masc=``he'', Fem=``she'', Neut=``it'' and Plur=``they''; ``Unk'' means the name was not found). The final column is the total count. The semantics of ``they$\vee$she'' is that the person accepts both ``they'' and ``she'' pronouns, while ``they$\wedge$she'' indicates that the person uses ``they'' or ``she'' depending on context (for instance, ``she'' while performing drag and ``they'' otherwise).}
\end{table}

The first question we ask is: what happens when this ``gender'' inference data is used to infer the gender of prominent non-binary individuals.
To this end, we took the names of $104$ non-binary people referenced on Wikipedia\footnote{\url{https://en.wikipedia.org/wiki/List_of_people_with_non-binary_gender_identities}, accessed Jan 5, 2019.} and queried the B+L data with them.
In almost all cases, the full name was unknown in the B+L data (or had counts less than five), and in which cases we backed off to simply querying on the given name.
We cross-tabulated the correct (according to Wikipedia) pronouns for these 90 people with the ``gender'' inferred by the B+L data.

The results are shown in \autoref{tab:bergsmawikinb}, where we can see that of those who use a pronoun other than \pron{she} or \pron{he} (exclusively) are, essentially always, misgendered.
Even in the best cases, the accuracy of this approach is only about $24\%$, and the errors occur much more frequently on pronouns other than \pron{he}.
This approach actively misgenders individuals, is harmful, and demonstrates that assigning gender to ``names'' does not work: anybody can have any combination of names and pronouns.


% The second question we ask, following on the observation by \citet{keyes2017names} that name-to-gender mappings may also encode a Western/European/White bias, is how well this resource generalizes across the world.
% To achieve this, we follow a similar paradigm to that proposed by \citet{buolamwini2018gender}, who used faces of world leaders to test skin-tone bias on facial recognition systems.
% Analogously, we test the ability of the B+L database to accurately categorize appropriate pronominal reference---and in this case, exclusively in binary gender categories---across the world.
% To do so, we collected the names of the current heads of state/government across the world according to Wikipedia at the beginning of 2006\footnote{\url{https://en.wikipedia.org/w/index.php?title=List_of_current_heads_of_state_and_government&oldid=33470304}} and in 2019\footnote{\url{https://en.wikipedia.org/w/index.php?title=List_of_current_heads_of_state_and_government&oldid=876260196}}, and tagged each of the approximately 250 world leaders according to the pronoun that Wikipedia uses to refer to them on their biographical page.\footnote{Using world leaders, rather than a random sample of names across the world, introduces its own bias: most of these are men, and most are from relatively high class and powerful families, and may have names that reflect that.}
% In the case that there were multiple heads of government/state, if \emph{one} of them used \pron{she} pronouns, we selected that person (because there are so few); otherwise we chose randomly.
% We then compare that pronoun with the results of querying their given name in the B+L dataset.
% The results are in \autoref{tab:world}.
% Here, we see that TODO.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "coref"
%%% End: 


==> lifecyclefig.tex <==

\newcommand{\arcarrow}[7]{%
% inner radius, middle radius, outer radius, start angle,
% end angle, tip protusion angle, options, text
  \pgfmathsetmacro{\rin}{#1}
  \pgfmathsetmacro{\rmid}{#2}
  \pgfmathsetmacro{\rout}{#3}
  \pgfmathsetmacro{\astart}{#4}
  \pgfmathsetmacro{\aend}{#5}
  \pgfmathsetmacro{\atip}{#6}
  \fill[#7] (\astart:\rin) arc (\astart:\aend:\rin)
    -- (\aend-\atip:\rmid) -- (\aend:\rout) arc (\aend:\astart:\rout)
    -- (\astart-\atip:\rmid) -- cycle;
%    \path[decorate] (\astart+\atip:\rmid) arc (\astart+\atip:\aend+\atip:\rmid);
  }

  \newcommand{\textconnectorwest}[2]{\draw[darkgreen!50!black,thick] ([yshift=-4]#2.north east) -- ([yshift=4]#2.south east) -- (#2.east) -- ([xshift=20]#2.east)  -- ([xshift=-20]#1.west) -- ([xshift=-2]#1.west);}
  
  \newcommand{\textconnectoreast}[2]{\draw[darkgreen!50!black,thick] ([yshift=-4]#2.north west) -- ([yshift=4]#2.south west) -- (#2.west) -- ([xshift=-20]#2.west) -- ([xshift=20]#1.east) -- ([xshift=2]#1.east);}


\begin{tikzpicture}[scale=0.9,
  node distance = 5mm and 5mm,
  lcstep/.style = {
    draw=white,
    very thick,
    top color=darkblue,
    bottom color=darkblue,
    rounded corners,
    text width=1.1cm,
    minimum height=1.1cm,
    minimum width=1.1cm,
    inner sep=0pt,
    align=flush center,
    text=white,
    font=\sffamily,
  },
  secref/.style = {
    rounded corners,
    draw=darkblue,
    very thick,
    top color=white,
    bottom color=darkblue!20,
    align=flush center,
    minimum width=0.8cm,
    font=\sffamily\footnotesize,
    inner sep=2pt,
  },
  extxtwest/.style = {
    align=flush right,
    font=\sffamily\footnotesize,
    anchor=east,
    text=darkgreen!50!black,
  },
  extxteast/.style = {
    align=flush left,
    font=\sffamily\footnotesize,
    anchor=west,
    text=darkgreen!50!black,
  },
  ]
  \linespread{0.8}

  \foreach \x in {0,4,...,360} {
    \arcarrow{2.35}{2.5}{2.65}{\x+1}{\x+3}{3}{darkblue!50,draw=darkblue!50}
  }
  \draw (90-0*360/8 : 2.5cm) node (def) [lcstep,double=darkblue,double distance=1pt] { Define\\Task };
  \draw (90-1*360/8 : 2.5cm) node (col) [lcstep] { Collect\\Data };
  \draw (90-2*360/8 : 2.5cm) node (lab) [lcstep] { Label\\Data };
  \draw (90-3*360/8 : 2.5cm) node (mod) [lcstep] { Define\\Model };
  \draw (90-4*360/8 : 2.5cm) node (tra) [lcstep] { Train\\Model };
  \draw (90-5*360/8 : 2.5cm) node (tst) [lcstep] { Test\\Model };
  \draw (90-6*360/8 : 2.5cm) node (dep) [lcstep] { Deploy\\Model };
  \draw (90-7*360/8 : 2.5cm) node (fbk) [lcstep] { Feed-\\back };

  \node at (def.south) [secref] {\autoref{sec:taskdef}};
  \node at (col.south) [secref] {\autoref{sec:datax}};
  \node at (lab.south) [secref] {\autoref{sec:datay}};
  \node at (mod.south) [secref] {\autoref{sec:model}};
  \node at (tst.south) [secref] {\autoref{sec:testing}};
  \node at (fbk.south) [secref] {\autoref{sec:feedback}};

  \node[extxteast] (coltxt) at ( 4.5,  2) { data excludes\\non-binary\\identities };
  \node[extxteast] (labtxt) at ( 4.5,  0) { annotator bias\\due to\\positionality/\\expectations };
  \node[extxteast] (modtxt) at ( 4.5, -2) { binary\\assumptions\\in features\\or constraints };

  \textconnectoreast{col}{coltxt}
  \textconnectoreast{lab}{labtxt}
  \textconnectoreast{mod}{modtxt}
  
  \node[extxtwest] (deftxt) at (-4.5,  2) { binary/or static\\gender assumptions };
  \node[extxtwest] (tsttxt) at (-4.5, -2) { evaluation\\that excludes\\true error costs };
  \node[extxtwest] (fbktxt) at (-4.5,  0) { active learning\\bootstrapping\\``gender'' dictionaries };
  
  \textconnectorwest{def}{deftxt}
  \textconnectorwest{tst}{tsttxt}
  \textconnectorwest{fbk}{fbktxt}

\end{tikzpicture}


==> taskdef.tex <==
Task definitions for linguistic annotations (like coreference) tend, in NLP, to be described in annotation guidelines (or, more recently, in datasheets or data statements \cite{gebru2018datasheets,bender2018data}).
These guidelines naturally change over the years as the community understands more and more about both the task and the annotation process (this is part of what makes the lifecycle a \textit{cycle}, rather than a pipeline).
Getting annotation guidelines ``right'' is \emph{difficult}, particularly in balancing informativeness with ability to achieve inter-annotator agreement, and \emph{important} because poorly defined tasks lead to a substantial amount of wasted research effort.


\noindent
\begin{table}
  \centering
  \tablesize
\begin{tabular}{llr} % {@{}l@{~~}l@{ }r@{}}
 \toprule
 \corpusname{LDC2001T02} & \corpusfullname{LDC2001T02} & {\scriptsize 2001T02} \\
 \corpusname{LDC2003T13} & \corpusfullname{LDC2003T13} & {\scriptsize 2003T13} \\
 \corpusname{LDC2005T09} & \corpusfullname{LDC2005T09} & {\scriptsize 2005T09} \\
 \corpusname{LDC2005T33} & \corpusfullname{LDC2005T33} & {\scriptsize 2005T33} \\
 \corpusname{LDC2006T06} & \corpusfullname{LDC2006T06} & {\scriptsize 2006T06} \\
 \corpusname{LDC2009T10} & \corpusfullname{LDC2009T10} & {\scriptsize 2009T10} \\
 \corpusname{LDC2009T26} & \corpusfullname{LDC2009T26} & {\scriptsize 2009T26} \\
 \corpusname{LDC2013T12} & \corpusfullname{LDC2013T12} & {\scriptsize 2013T12} \\
 \corpusname{LDC2013T19} & \corpusfullname{LDC2013T19} & {\scriptsize 2013T19} \\
 \corpusname{LDC2014T18} & \corpusfullname{LDC2014T18} & {\scriptsize 2014T18} \\
 \corpusname{LDC2017T10} & \corpusfullname{LDC2017T10} & {\scriptsize 2017T10} \\
 \corpusname{GAP}        & \corpusfullname{GAP}        & \hspace{-40mm}{\scriptsize \citet{webster2018mind}} \\
 \corpusname{QB}         & \corpusfullname{QB}         & \hspace{-40mm}{\scriptsize \citet{guha2015removing}} \\
 \bottomrule
\end{tabular}
\caption{\label{tab:corpora}Corpora analyzed in this paper.}
\end{table}

For the purposes of this study, we consider here (and elsewhere in this paper) thirteen datasets on which coreference or anaphora are annotated in English (\autoref{tab:corpora}); eleven of these are corpora distributed by the Linguistic Data Consortium (LDC)\footnote{See \url{https://catalog.ldc.upenn.edu/{LDC-ID}}.}, and two are not.
The final non-LDC corpora do not (to our knowledge) have corresponding annotation guidelines, and are instead described in associated papers.
None of the annotation guidelines (or papers) give explicit guidance about what personal pronouns are to be considered, or otherwise what information a human annotator should use to resolve ambiguous situations.
However, many of them do provide running \emph{examples}, which we can analyze.

To assess task definition bias, we count, for each of the annotation guidelines, how many examples use different pronominal forms.
For examples that use \pron{they}, we separate four different subtypes, following \citepos{conrod2018agree} categorization (see \autoref{sec:linggender}):
\begin{enumerate}
  \item[\pron{nh}:] Plural non-human group -- ``The knives are put away in their carrier.''
  \item[\pron{pl}:] Plural group of humans -- ``The children are friendly, and they are happy.''
  \item[\pron{qi}:] Quantified/indefinite -- ``Most chefs harshly critique their own dishes.''
  \item[\pron{sp}:] Specific singular referent -- ``Jun enjoys teaching their students.''
\end{enumerate}

\noindent
The results are shown in \autoref{tab:annotation} (datasets for which no relevant examples were provided are not listed).
Overall, we see that in total across these seven datasets, examples with \pron{he} occur more than twice as frequently as all others combined.
Furthermore, \pron{they} is never used in a specific setting and, somewhat interestingly, is only used as an example for quantification in \emph{older} datasets (2005 and before).
Moreover, none of the annotation guidelines have examples using neopronouns.
This lack does nothing to counterbalance a general societal bias that tends to erase non-binary identities.
In the case of GAP, it is explicitly mentioned that that \emph{only} \pron{she} and \pron{he} examples are considered (and only in cases where the gender of two possible referents ``matches''---though it is unspecified what type of gender this is and how it is determined).
Even on the binary spectrum, there is also an obvious gender bias between \pron{he} and \pron{she} examples.

%we consider the following questions for each dataset, building on and extending \citep{keyes18misgendering} survey of computer vision papers on the topic of gender recognition of faces.
%\begin{enumerate}
%\item do the guidelines distinguish grammatical from social gender?
%\item do the guidelines assume social gender is binary?
%\item do the guidelines allow for neopronouns or singular they?
%\item do the guidelines assume that gender (of any kind) is immutable?
%\end{enumerate}
%most likely for most of these questions the answer will be ``not at all addressed'' so it's worth keeping three answers ``yes'', ``no'' and ``not discussed''

\begin{table}
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \renewcommand{\arraystretch}{1.0}
  \tablesize\centering
  \begin{tabular}{l@{\qquad}ggg@{\qquad}cccc}
    \toprule
    &&&& \multicolumn{4}{c}{\pron{they}} \\[0em]
    & \pron{she}
    & \pron{he}
    & \pron{neo}
    & \pron{sp}
    & \pron{qi}
    & \pron{pl}
    & \pron{nh}
    \\
    \midrule %               SHE HE  NEO -SP -Q  -P  -NH
    \corpusname{LDC2001T02} &   &~~7 &   &   & 2 & 1 &   \\
    % does not discuss gender at all; does not specify which pronouns count beyond "first second and third"; does not say antyhing about neopronouns/sthey
    % 3rd person pronouns the refer to people in examples: he*7, they-pgroup*1, they+quant*2 ("Most computational linguists prefer _their_ own parsers.", "Every man who knows his own mind", ...)
    \corpusname{LDC2003T13} &   &~~4 &   &   & 3 &   &   \\
    % he*4, they+quant*3 (same)
    \corpusname{LDC2005T09} & 2 &~~6 &   &   & 1 &   &   \\
    % he*6, she*2, they+quant ("They are not lawyers"), they (context-free)
%   \corpusname{LDC2005T33} &   &   &   &   &   &   &   \\
    % nothing
%   \corpusname{LDC2006T06} &   &   &   &   &   &   &   \\
    % nothing
    \corpusname{LDC2009T10} & 1 &~~2 &   &   &   &   &   \\
    % he*2, her*1
%   \corpusname{LDC2009T26} &   &   &   &   &   &   &   \\
    % nothing
%   \corpusname{LDC2013T12} &   &   &   &   &   &   &   \\
    % nothing
    \corpusname{LDC2013T19} & 1 &   &   &   &   &   &   \\
    % she*1, 
%   \corpusname{LDC2014T18} &   &   &   &   &   &   &   \\
    % nothing
    \corpusname{LDC2017T10} & 5 &17 &   &   &   &   &   \\
    % he*17, she*5, they+unk*4
%   GAP                     &   &   &   &   &   &   &   \\
    % "GAP   examples   are   not   strictly   Winogradschemas because they have no reference-flippingword.Nonetheless,   they  contain  two  personnamed  entities  of  the  same  gender  and  an  am-biguous pronoun that may refer to either (or nei-ther). "
    % she*6, he*5
    QB                      &   &~~1 &   &   &   &   &   \\
    % they+unk, he*1,
    % some examples that obscure gender eg "This writer..." "That title character ...", ...
    \midrule
    \textbf{Total}          & 9 & 37& 0 & 0 & 6 & 1 & 0 \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:annotation}  Frequency counts of different pronouns in example annotations given in annotation instructions for seven of the datasets that provide examples. Zeros are omitted from the table. \emph{No datasets contain examples using neopronouns, nor any examples using ``they'' to refer to a singular specific entity (and only older datasets included any examples of quantified usages of ``they'').}}
\end{table}
    
                        
  



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "coref"
%%% End: 


==> testing.tex <==
Bias can also show up at testing time, due either to data or metrics.
For instance, if one evaluates on highly biased data, it will be difficult to capture disparities (akin to the over-representation of light skinned men in computer vision datasets~\citep{buolamwini2018gender}).
Alternatively, evaluation metrics may weight different errors in a way that is incongruous with their harm.
For example, while misgendering via the use of an incorrect pronoun is a high cost social error \citep{stryker08transgender}, evaluation metrics may or may not reflect the true cost of such mistakes.

In terms of data, most coreference resolution systems are evaluated intrinsically, by testing them against gold standard annotations using a variety of metrics; in this case, all the observations on data bias (\autoref{sec:datax} and \autoref{sec:datay}) apply.
Sometimes coreference resolution is used as part of a larger system.
For instance, information retrieval can use coreference resolution to help accurately rank documents by up-weighting the importance of entities that are referred to frequently~\citep{du1990anaphora,pirkola1996effect,edens2003investigation}.
In machine translation, producing correct gendered forms in gender languages often requires coreference to have been solved~\citep{mitkov1999introduction,hardmeier2010modelling,guillou2012improving,hardmeier2018pronoun}.
In the translation case, this then begs the question: which data are being used and how biased are they?
It turns out, ``quite biased.''
Even limiting to just \pron{she} and \pron{he} pronouns, the bias is significant: four times as many \pron{he} than \pron{she} in Europarl~\citep{koehn2005europarl} and the Common Crawl~\citep{smith2013dirt}, six times as many in News Commentaries~\citep{tiedemann2012opus}, and fifty times as many in Hong Kong Laws corpus.

In terms of metrics, most intrinsic evaluation is carried out using metrics like MUC~\citep{vilain1995model}, ACE~\citep{mitchell2005ace}, B$^3$~\citep{bagga1998algorithms,stoyanov2009conundrums}, or CEAF~\citep{luo2005coreference} (see also \citep{cai2010evaluation} for additional discussion and variants).
As observed by \citet{agarwal2019evaluation}, most of these metrics are rather insensitive to arguably large errors, like the inability to link pronouns to names; to address this, they introduce a new metric to focus specifically on this named entity coreference task.
These metrics also generally treat all errors similarly, regardless of whether the error compounds societal injustices (e.g., ignoring an instance of \pron{xyr}) or not (e.g., ignore an instance of \pron{he}), despite the fact that these have vastly different implications from the perspective of justice \citep[e.g.,]{fraser2008abnormal}.

% \begin{table}
%   \centering\tablesize
%   \begin{tabular}{lccc}
%     \toprule
%     & \textbf{Bleu} & \textbf{Bleu} & \\
%     \textbf{Dataset} & \textbf{Overall} & \textbf{Pro-Only} & \textbf{Pro \%}\\
%     \midrule
%         wmt18     & 99.1 & 95.4 & 17.7 \\    % et-en
%         wmt17     & 99.0 & 95.1 & 18.1 \\    % cs-en
%         wmt16     & 99.4 & 97.4 & 19.0 \\    % cs-en
%         wmt15     & 98.9 & 95.1 & 19.7 \\    % cs-en
%         wmt14     & 99.4 & 97.2 & 20.8 \\    % hi-en
%         wmt13     & 99.7 & 98.4 & 14.0 \\    % de-en
%         wmt12     & 99.3 & 97.0 & 19.6 \\    % de-en
%         wmt11     & 99.5 & 97.5 & 17.4 \\    % de-en
%         wmt10     & 99.5 & 97.8 & 19.0 \\    % es-en
%         wmt09     & 99.5 & 97.1 & 15.8 \\    % de-en
%         wmt08     & 99.7 & 98.3 & 14.5 \\    % fr-en
%         iwslt17   & 99.6 & 95.0 & ~~6.5 \\    % fr-en
%     \midrule
%     \textbf{average} & 99.4 & 96.9 & 16.8 \\
%     \bottomrule
%   \end{tabular}
%   \caption{\label{tab:bleu} \hal{cut?} Bleu scores on various machine translation datasets with entirely \pron{he} pronoun sets. Rows are datasets. Columns are: overall Bleu score when \pron{she} is replaced with \pron{he}; Bleu score evaluated just on sentences with \pron{she} or \pron{he} pronouns; percentage of such sentences.}
% \end{table}
    
For extrinsic evaluation, the metrics used are those that are appropriate for the downstream task (e.g., machine translation).
In the case of machine translation, folk lore has it that getting pronouns ``correct'' does not really impact Bleu scores, which was recently confirmed (and alternatives proposed) by \citet{guillou2018automatic}.
To quantify this bias, we use the sacreBLEU toolkit~\citep{post2018call} and compute Bleu scores between the ground truth reference outputs and those same references where all \pron{she} pronouns were replaced with morphologically equivalent \pron{he} forms (none of these datasets contain neopronouns and analysis of a small sample did not find any singular specific uses of \pron{they}).
From wmt08--wmt18 and iwslt17 test sets, the average percentage \emph{drop} in Bleu score from this error is $0.67\%$ ($\pm 0.22$), which is barely statistically significant.
Evaluated only on the $\approx 17\%$ of the sentences in these datasets containing either \pron{he} or \pron{she}, the degradation is about $3.1\%$.
While this degradation is noticable, it perhaps does not reflect the real cost of such translation errors due to the high societal cost of misgendering.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "coref"
%%% End: 

